Mumford-Shah regularization in electrical impedance tomography with complete electrode model

In electrical impedance tomography, we aim to solve the conductivity within a target body through electrical measurements made on the surface of the target. This inverse conductivity problem is severely ill-posed, especially in real applications with only partial boundary data available. Thus regularization has to be introduced. Conventionally regularization promoting smooth features is used, however, the Mumford--Shah regularizer familiar for image segmentation is more appropriate for targets consisting of several distinct objects or materials. It is, however, numerically challenging. We show theoretically through $\Gamma$-convergence that a modification of the Ambrosio--Tortorelli approximation of the Mumford--Shah regularizer is applicable to electrical impedance tomography, in particular the complete electrode model of boundary measurements. With numerical and experimental studies, we confirm that this functional works in practice and produces higher quality results than typical regularizations employed in electrical impedance tomography when the conductivity of the target consists of distinct smoothly-varying regions.

==> Figures/Layout/Case2.tex <==
\captionsetup[subfloat]{position=top,labelformat=empty}
\begin{figure*}[!t]%
\centering%
\begin{minipage}{0.85\textwidth}%
    \subfloatcolorbar{0.0cm}{-4.8cm}{0.118\textwidth}{"Figures/Case0/CBz".png}%    
    \centering%
        \rotatebox{90}{\hspace{-4.0cm} $F_\lambda,z$ \hspace{2.3cm} $F_\lambda,\gamma$ \hspace{2.9cm} TV}
        \subcstaged{$a = 10^{-1}$}{$\alpha = 10^{-3}$}{"Figures/Case2/Disk16_TV_c2_3".png}{"Figures/Case2/Disk16_Case2_2".png}{"Figures/Case2/Disk16_Case2_2z".png}{130}{130}{130}{130}%
        \subcstaged{$a = 1$}{$\alpha = 10^{-2}$}{"Figures/Case2/Disk16_TV_c2_4".png}{"Figures/Case2/Disk16_Case2_3".png}{"Figures/Case2/Disk16_Case2_3z".png}{130}{130}{130}{130}%
        \subcstaged{$a = 10$}{$\alpha = 10^{-1}$}{"Figures/Case2/Disk16_TV_c2_5".png}{"Figures/Case2/Disk16_Case2_4".png}{"Figures/Case2/Disk16_Case2_4z".png}{130}{130}{130}{130}%
        %\subcstageb{Stage 4.}{sfig:c2s4}{0.18\linewidth}{"Figures/Case1/Chamber5_w1s".png}{"Figures/Case1/Chamber5_w1".png}{200}{50}{200}{200}%                  
    \end{minipage}% 
    \hspace{-1.35cm}
    \subfloatcolorbar{0.0cm}{-4.8cm}{0.1005\textwidth}{"Figures/Case0/CB".png}%    
    \caption{Case 2. Comparison of $F_\lambda$ and $\TV$. Top row: $\TV$ regularised solution. Middle and bottom rows: $F_\lambda$ regularised solutions of $\gamma$ and $z$. The control parameter is $\lambda = 10^{-3}$.}%
    \label{fig:Case2}%
\end{figure*}%
\captionsetup[subfloat]{position=bottom}

